Adaptive Private-K-Selection with Adaptive K and Application to Multi-label PATE

We provide an end-to-end Renyi DP based-framework for differentially private top-$k$ selection. Unlike previous approaches, which require a data-independent choice on $k$, we propose to privately release a data-dependent choice of $k$ such that the gap between $k$-th and the $(k+1)$st "quality" is large. This is achieved by a novel application of the Report-Noisy-Max. Not only does this eliminate one hyperparameter, the adaptive choice of $k$ also certifies the stability of the top-$k$ indices in the unordered set so we can release them using a variant of propose-test-release (PTR) without adding noise. We show that our construction improves the privacy-utility trade-offs compared to the previous top-$k$ selection algorithms theoretically and empirically. Additionally, we apply our algorithm to "Private Aggregation of Teacher Ensembles (PATE)" in multi-label classification tasks with a large number of labels and show that it leads to significant performance gains.

==> related_work.tex <==
\section{Related Work}




% For report noisy max part: compare ours with exponential mechanism
% for k selection
%\subsection{Comparison with data-dependent RDP}
%\citet{papernot2018} propose the data-dependent RDP analysis for the report noisy max mechanism ($k=1$ in our case ). Their algorithm consists of the report noisy max composition, where a fixed noise is injected into each query, and the data-dependent privacy cost is adapted to the vote margin within each query. Our algorithm can be applied to this query release problem in an alternative way: fixing each query's privacy budget while adaptively adjusting the noise scale based on the smooth sensitivity. In short, the data-dependent RDP analysis is ``privacy-first'' while ours is ``accuracy first''.



